Towards User-Driven Neural Machine Translation

A good translation should not only translate the original content semantically, but also incarnate personal traits of the original text. For a real-world neural machine translation (NMT) system, these user traits (e.g., topic preference, stylistic characteristics and expression habits) can be preserved in user behavior (e.g., historical inputs). However, current NMT systems marginally consider the user behavior due to: 1) the difficulty of modeling user portraits in zero-shot scenarios, and 2) the lack of user-behavior annotated parallel dataset. To fill this gap, we introduce a novel framework called user-driven NMT. Specifically, a cache-based module and a user-driven contrastive learning method are proposed to offer NMT the ability to capture potential user traits from their historical inputs under a zero-shot learning fashion. Furthermore, we contribute the first Chinese-English parallel corpus annotated with user behavior called UDT-Corpus. Experimental results confirm that the proposed user-driven NMT can generate user-specific translations.

==> backup.tex <==
%\subsection{Overview}
%Figure xx illustrates the model architecture. Compared with the traditional transformer-based NMT model~\cite{vaswani2017attention}, the proposed model involves two new components: 1) a cache module for user behavior modeling as described in \S~\ref{sec:cache}; 2) the contrastive learning to decrease the divergence between translations of similar users while increasing the diversity on dis-similar users as described in \S~\ref{sec:contra}. 

%As mentioned in \S~\ref{sec:problem}, for user-driven NMT, the translation of a source sentence under the user trait information $u$ is given by:
%\begin{equation}
%    P(Y^{(u)}|X^{(u)},u;\theta)=\prod_t P(y_{t}^{(u)}|X^{(u)},Y_{<t}^{(u)},u;\theta).
%\end{equation}
%To be concrete, the historical inputs of the users are used as $u$ to represent the user behaviors as we discussed in \S~\ref{sec:intro}. 
%The translation loss can be written as: 
%\begin{equation}
%\mathcal{L}_{\textrm{MLE}}=\sum_{t}-\log P(y_{t}^{(u)}|X^{(u)},Y_{<t}^{(u)},u;\theta).
%\end{equation}

\iffalse
\subsection{Cache-based User Behavior Modeling}\label{sec:cache}

%Since the current NMT models generate the translation in the word-by-word manner, we argue that the user trait can also be represented at word level, 
For the user behavior modeling, we further incorporate the cache mechanism into the NMT model. With the goal of modeling user behavior, we hope that the cache should be designed to represent the domain signal and context information. Specifically, we represent the user behavior at the word level based on the historical input. Two kinds of keywords are extracted from the historical input, including the topic keywords for the domain signal capturing, and the context keywords to capture the information of the recent input context. 

We define the topic cache $M$ and the context cache $N$ of $u$ as series of keyword embeddings, which contains topic keyword embeddings $m^{(u)}$ and context keyword embeddings $n^{(u)}$:
%To capture user behavior and generate personalized translation, we propose to augment NMT model with two cache modules: topic cache $M$  and context cache $N$.
\begin{equation}
    M^{(u)}=\left[m^{(u)}_1,m^{(u)}_2,...,m^{(u)}_{|M^{(u)}|}\right],
\end{equation}
\begin{equation}
    N^{(u)}=\left[n^{(u)}_1,n^{(u)}_2,...,n^{(u)}_{|N^{(u)}|}\right],
\end{equation}
here we use $|\cdot|$ to denote the length.

Given a user, we first initialize the topic cache and the context cache according to the historical inputs and the current source input, where the details are described in \S~\ref{sec:init}. Furthermore, for the online NMT system, when the user inputs a new sentence, the cache module will be updated as described in \S~\ref{sec:update}. After that, given the topic cache $M$ and the context cache $N$, we obtain the corresponding cache vector $c^{(u)}$ by taking an average pooling over them: 

\begin{equation}
    c^{(u)}=\frac{1}{|M^{(u)}|+|N^{(u)}|}\left(\sum m^{(u)}+\sum n^{(u)}\right),
\end{equation}

\begin{equation}
    c^{(u)}=\textrm{MeanPooling}\left(\left[M^{(u)};N^{(u)}\right]\right),
\end{equation}
where $[\cdot;\cdot]$ denotes the  operation of concatenation.

Given the original source input embeddings $ X^{(u)}=\{x_1^{(u)},...,x_{|X^{(u)}|}^{(u)}\}$, the cache vector is introduced into them in the following way\footnote{Note that in our preliminary experiments, we also tried to use the attention mechanism to fuse the cache vector into the NMT model, but no better performance was obtained.}:
\begin{equation}
    \hat{X}^{(u)}=\{x_1^{(u)} + c^{(u)},...,x_{|X^{(u)}|}^{(u)}+c^{(u)}\}.
\end{equation}
  
The model then use source embedding $\hat{X}^{(u)}$ augmented with user traits to generate personalized translations. 


\subsubsection{Cache Initialization}
\label{sec:init}
For each user, we initialize the cache in the following ways. Firstly, we use the TF-IDF to identify the topic keywords and the context keywords from the historical inputs $H^{(u)}$ and current source input $X^{(u)}$. %calculate the TF-IDF value of each word in the vocabulary and obtain a history TF-IDF vector $v^{(u)}_m$ and a current input TF-IDF vector $v^{(u)}_n$, of which each grid represents the TF-IDF value of the corresponding word in the historical inputs and the current source input, respectively. 
Note that for the original definition of TF-IDF, its calculation involves the word $w$ to be calculated, the document $d$ containing $w$, and the corpus $D$ containing $d$, which can be formulated as:
\begin{equation}
\textrm{TF-IDF}(w, d, \mathcal{D})=\textrm{TF}(w, d)\times \textrm{IDF}(w, d, \mathcal{D}),
\end{equation}
%where
%\begin{equation}
%\textrm{TF}(w, d)=\frac{|w\in d|}{\textrm{count}(d)},
%\end{equation}
%and 
%\begin{equation}
%\textrm{IDF}(w, d, \mathcal{D})=\log(\frac{|\mathcal{D}|}{|d\in{D}:w\in{d}|+1}),
%\end{equation}
where
\begin{equation}
\textrm{TF}(w, d)=\frac{\textrm{count}(w, d)}{\sum_{w' \in d}{\textrm{count}(w', d)}},
\end{equation}
and
\begin{equation}
\textrm{IDF}(w, d, \mathcal{D})=\log\left(\frac{\sum_{w' \in \mathcal{D}}{\textrm{count}(w', \mathcal{D})}}{\textrm{count}(w, d)+1}\right),
\end{equation}
here we use the notation $\textrm{count}(w, \mathcal{D})$ to denote the number of occurrences of the word $w$ in corpus $\mathcal{D}$. %and $count(*)$ calculate the total word number of the input. 

%By picking the grid with value higher than the threshold $\gamma$, we can get the topic keywords and the context keywords. 
Since the topic cache aims at capturing the global and long-term user features, when calculating the TF-IDF($w, d, \mathcal{D}$) for topic keyword selection, we treat the historical inputs as the ``document'' $d$ and the historical inputs of all users in the corpus are regarded as $\mathcal{D}$. The TF-IDF weight of each word $w$ can be calculated as:
\begin{equation}
    \textrm{TF-IDF}(w, H^{(u)}, H^{(\mathcal{D})}).
\end{equation}
where $H^{(\mathcal{D})}$ denotes the the historical inputs of all users in the corpus. We select the words as the topic keywords whose TF-IDF weight is higher than a predefined threshold.
Different from the topic cache, the context cache aims at capturing the short-term features. Therefore, for a current input source $X^{(u)}$, the TF-IDF weight of each word $w$ is calculated as:
\begin{equation}
   \textrm{TF-IDF}\left(w, X^{(u)}, H^{(u)}\right).
\end{equation}

Furthermore, for the user without historical inputs, we find the closest user $u^+$ according to the cosine similarities between their topic keywords TF-IDF vector $v^{(u)}_m$, and initialize the topic cache with the topic keywords of $u^+$.
Finally, we store the embeddings of these keywords in the topic cache and the context cache, respectively. 


\subsubsection{Cache Updating}
\label{sec:update}
For the online MT system, the users tend to continuously inputting new sentences, thus the cache should be dynamically updated.
For the topic cache, we re-calculate the TF-IDF and update all the words in cache. %since we want the topic cache to represent the topic word of current user. As 
For the context cache, we use first-in-first-out rule to replace those words that occur earlier. We can also consider context cache as a ``filter window'' that slides cross previous source inputs.
\fi

\iffalse
We use cache to represent user personality. For each user $i$, the user embedding at time $t$ is:
\begin{equation}
    e^i_t={ch}^i_t+{cc}^i_t
\end{equation}
The query list is initialized as:
\begin{equation}
    q^i_0=X^i_h
\end{equation}
$X^i_h$ are all historical input sentences of user $i$. $q^i$ is Updated as:
\begin{equation}
    q^i_t=q^i_{t-1}+x^i_t
\end{equation}
The words $w$ to initialize topic cache are selected by:
\begin{equation}
    \mathbf{tf-idf}(w, x^i_0, q^i_0)
\end{equation}
When updating the topic cache at time $t$, for each word $w$ in query sentence $x^i_t$, we have: 
\begin{equation}
    \mathbf{tf-idf}(w, x^i_t, \sum_{i\in{U}}q^i_t)
\end{equation}
$U$ is the set containing all users.
As for the context cache of user i, for each word w in query sentence d, we have: 
\begin{equation}
    \mathbf{tf-idf}(w, x^i_t, q^i_{t-1})
\end{equation}


\subsection{Contrastive Learning}
\label{sec:contra}
In user-driven NMT, each user contains few annotated sentences, which makes it difficult to learn diversity in translation across different users. For a user $u$, given the same source input $X^{(u)}$ but similar user $u^{+}$, the model should generate similar translation, and generate dissimilar translation of $X^{(u)}$ for dissimilar user $u^{-}$ conversely. 
Therefore, in response to the problem of few-shot samples, we can use the output of $u^{+}$ and $u^{-}$ to construct the positive and negative sample, respectively. 
Specifically, we define the similarity score of two users $u_1$ and $u_2$ with the cosine similarity of their topic keywords TF-IDF vectorss $v^{(u)}_m$ as:
\begin{equation}
    \textrm{score}(u_1,u_2)=\frac{v^{(u_1)}_m  v^{(u_2)}_m}{||v^{(u_1)}_m||\cdot||v^{(u_2)}_m||}
\end{equation}
For each user $u$, we select the user with the highest similarity score as positive sample $u^+$ for faithfulness, and randomly pick the user with $\textrm{score}(u, u^-)=0$ as contrastive sample for diversity. 
We employ contrastive learning where the translation of similar users and dissimilar users are considered as positive and contrastive samples.
Our contrastive learning approach is equipped with a triplet-margin loss. 
The triplet-margin loss ensures that the margins of the log-likelihood distance between the $\langle$ground-truth, positive$\rangle$ pairs and the $\langle$ground-truth, negative$\rangle$ pairs are higher than the setting $\eta$:
\iffalse
\begin{align}
\mathcal{L}_{\textrm{CL}}=\sum_{u=1}^U[||\log P(y_{t}|X^{(u)},Y_{<t},u)\\
-\log P(y_{t}^+|X^{(u)},Y^+_{<t},u^+)||^2_2+\eta\\
-||\log P(y_{t}^+|X^{(u)},Y_{<t},u)\\
-\log P(y_{t}^-|X^{(u)},Y^-_{<t},u^-)||^2_2,0]\nonumber
\end{align}
\fi

\begin{equation}
    \mathcal{L}_{\textrm{CL}}=\sum_{u=1}^U[\textrm{dis}(u,u^+)-\textrm{dis}(u,u^-)+\eta,0]
\end{equation}
\begin{align}
    \textrm{dis}(u,u^+)=||\log P(y_{t}^+|X^{(u)},Y_{<t},u)\\-\log P(y_{t}^+|X^{(u)},Y^+_{<t},u^+)||^2_2
\end{align}
\begin{align}
    \textrm{dis}(u,u^-)=||\log P(y_{t}^+|X^{(u)},Y_{<t},u)\\-\log P(y_{t}^+|X^{(u)},Y^+_{<t},u^+)||^2_2
\end{align}

%\begin{align}
%\mathcal{L}_{\textrm{CL}}=\sum_{u=1}^U \max (\Delta - \log P(y_{t}^+|X^{(u)},Y^+_{<t},u^+) + \\ \log P(y_{t}^-|X^{(u)},Y^-_{<t},u^-),0)\nonumber
%\end{align}
By narrowing the text prediction distribution of similar user and conversely generating more diverse translations for dissimilar user, our model can generate translation more in line with user traits. 
The final loss of our model is the combination of two losses:
\begin{equation}
    \mathcal{L}=\mathcal{L}_{\textrm{MLE}}+\mathcal{L}_{\textrm{CL}}.
\end{equation}
\fi

